DetCLIPv2: Scalable Open-Vocabulary Object Detection Pre-training via Word-Region Alignment

This paper presents DetCLIPv2, an efficient and scalable training framework that incorporates large-scale image-text pairs to achieve open-vocabulary object detection (OVD). Unlike previous OVD frameworks that typically rely on a pre-trained vision-language model (e.g., CLIP) or exploit image-text pairs via a pseudo labeling process, DetCLIPv2 directly learns the fine-grained word-region alignment from massive image-text pairs in an end-to-end manner. To accomplish this, we employ a maximum word-region similarity between region proposals and textual words to guide the contrastive objective. To enable the model to gain localization capability while learning broad concepts, DetCLIPv2 is trained with a hybrid supervision from detection, grounding and image-text pair data under a unified data formulation. By jointly training with an alternating scheme and adopting low-resolution input for image-text pairs, DetCLIPv2 exploits image-text pair data efficiently and effectively: DetCLIPv2 utilizes 13X more image-text pairs than DetCLIP with a similar training time and improves performance. With 13M image-text pairs for pre-training, DetCLIPv2 demonstrates superior open-vocabulary detection performance, e.g., DetCLIPv2 with Swin-T backbone achieves 40.4% zero-shot AP on the LVIS benchmark, which outperforms previous works GLIP/GLIPv2/DetCLIP by 14.4/11.4/4.5% AP, respectively, and even beats its fully-supervised counterpart by a large margin.

==> latex_files/experiments.tex <==
\vspace{-2mm}
\section{Experimental Results}
\label{subsec:Experimental Results}

\subsection{Implementation Details}\label{subsec:implementation_detail}
\vspace{-1mm}
\paragraph{Training Dataset.} We use multiple datasets from different sources for training (Table~\ref{tab:dataset_info}). Specifically, for detection data, we use a sampled subset from Objects365v2 \cite{shao2019objects365} dataset (denoted as O365) with 0.66M images; for grounding data, we use GoldG \cite{kamath2021mdetr} with COCO \cite{Lin2014coco} images removed, which results in a fairer zero-shot evaluation on LVIS \cite{gupta2019lvis}. For image-text pairs, we use 2 versions of Conceptual Captions (CC) datasets, i.e., CC3M \cite{sharma2018conceptual} and CC12M \cite{changpinyo2021cc12m} (together denoted as CC15M). 

% training dataset information
\begin{table}[t]
\centering
\vspace{-.5em}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcc}
\toprule
Dataset & Type & Volume \\
\midrule 
Objects365 \cite{shao2019objects365} (O365)  & Detection & 0.66M  \\
GoldG \cite{kamath2021mdetr} &Grounding & 0.77M  \\
\makecell[l]{CC15M \\(CC3M \cite{sharma2018conceptual}+CC12M \cite{changpinyo2021cc12m})} & Image-text pairs  & \makecell[c]{13M \\ (3M+10M)}  \\
\bottomrule
\end{tabular}
}
\vspace{-.7em}
\caption{A summary of training data. CC15M contains only 13M image-text pairs since some urls are invalid.}
\vspace{-1em}
\label{tab:dataset_info}
\end{table}

%############################################################################################
\paragraph{Training details.} We use Swin-transformer \cite{liu2021swin} backbones for image encoder. For text encoder, the maximum token length is set to 16 for efficient training and inference. We initialize the text-encoder with a pretrained FILIP model \cite{yao2021filip}. 32/64 V100 GPUs are used for training Swin-T/L-based models, respectively. For detection and grounding data, we use input resolution $1333\times800$ with a batch size of 128/256 for Swin-T/L models (4 per card), respectively; and for image-text pairs, we use input resolution $320\times320$ with a batch size of 6144 (192/96 per card for Swin-T/L model). We set $\alpha=2$ and  $\beta=1$ and $\lambda=0.1$ in Eq.~\ref{eq:overall_objectives}. Without otherwise specified, all models are trained with 12 epochs. More training details can refer to Appendix.

\paragraph{Evaluation benchmark.}
Following GLIP \cite{li2021grounded} and DetCLIP \cite{yao2022detclip}, we evaluate our method's \textit{zero-shot} performances on LVIS \cite{gupta2019lvis} with 1203 categories. \textit{Fixed} AP \cite{dave2021evaluating} on LVIS minival5k are reported for ablation and comparison with other methods. To further study the generalization ability of our method, we also evaluate with ODinW13 dataset \cite{li2021grounded,zhang2022glipv2}, which contains 13 downstream detection tasks with highly varied distributions. We focus on the GLIP protocol \cite{li2021grounded} rather than the ViLD protocol \cite{gu2021open} that splits LVIS into seen/unseen categories, since the former is a stronger and more practical open-world setting that does not make any prior assumptions on downstream tasks while the latter still requires partial LVIS data for training.

% ######################### Ablation studied #############################
\vspace{-1mm}
\subsection{Ablation Studies}\label{subsec:ablation_study}
\vspace{-1mm}
%##########################################################################
%overall table of contrastive learning ablations 
\begin{table*}[t]
\vspace{-4mm}
\centering
%#################################################
% proposal selection strategy
%#################################################
\subfloat[
\textbf{Proposal selection strategy}. Batch-wised text similarity generates better proposals for contrastive learning.
\label{tab:proposal_selection}
]{
\centering
\begin{minipage}{0.29\linewidth}{\begin{center}
\tablestyle{4pt}{1.05}
\begin{tabular}{lcc}
\# & Strategy & AP (r/c/f)\\
\shline
1 & cls  & 28.4 (26.6/28.2/28.8)    \\
2 & IoU & 30.1 (30.0/30.1/30.2)   \\
3 & centerness & 30.2 (28.4/30.6/30.1)   \\
4 & text sim (S) &  29.6 (24.9/29.5/30.5) \\
5 & text sim (B) & \baseline{\textbf{31.3} (29.4/\textbf{31.7}/\textbf{31.3})} \\
6 & \makecell[c]{text sim (B) + \\ centerness} & 30.9 (\textbf{30.2}/31.1/30.8) \\
\end{tabular}
\end{center}}\end{minipage}
 }
\hspace{2em}
%#################################################
% num of proposals
%#################################################
\subfloat[
\textbf{Number of proposals}. Using 100 proposals per image works the best.
\label{tab:number_proposals}
]{
\begin{minipage}{0.29\linewidth}{\begin{center}
\tablestyle{6pt}{1.05}
\begin{tabular}{cc}

top-k & AP (r/c/f) \\
\shline
25 & {30.6 (29.9/30.5/30.8)} \\
50 & {30.8 (\textbf{30.2}/30.6/31.0)} \\
100 & \baseline{\textbf{31.3} (29.4/\textbf{31.7}/\textbf{31.3})}  \\
200 & {30.8 (29.4/30.6/31.1)}  \\
\multicolumn{2}{c}{~}\\
\multicolumn{2}{c}{~}\\
\multicolumn{2}{c}{~}\\
\end{tabular}
\end{center}}\end{minipage}
}
\hspace{2em}
%#################################################
% contrastive loss design
%#################################################
\subfloat[
\textbf{Contrastive loss design}. Excluding image-to-text contrastive loss can boost the performance.
\label{tab:contrastive_loss}
]{
\begin{minipage}{0.29\linewidth}{\begin{center}
\tablestyle{4pt}{1.05}
\begin{tabular}{cc}
Design & AP (r/c/f)\\
\shline
text-to-image & \baseline{\textbf{31.3} (29.4/\textbf{31.7}/\textbf{31.3})}  \\
image-to-text & {29.8 (\textbf{30.0}/29.7/29.9)} \\
bilateral & {30.9 (\textbf{30.0}/31.5/30.5)} \\
\multicolumn{2}{c}{~}\\
\multicolumn{2}{c}{~}\\
\multicolumn{2}{c}{~}\\
\multicolumn{2}{c}{~}\\
\end{tabular}
\end{center}}\end{minipage}
}
\\
\centering
\vspace{.3em}
%#################################################
% Word-region alignment strategy
%#################################################
\subfloat[
\textbf{Word-region matching strategy}. Matching each textual concept to the closest region is effective and memory-efficient.
\label{tab:matching_strategy}
]{
\centering
\begin{minipage}{0.29\linewidth}{\begin{center}
\tablestyle{1.5pt}{1.05}
\begin{tabular}{lccc}
\# &Strategy & AP (r/c/f) & Memory\\
\shline
1 & max-bbox & {29.8 (28.5/39.5/30.4)} &  19.8 GB \\
2 & 1-to-1 & \baseline{\textbf{31.3} (29.4/\textbf{31.7}/\textbf{31.3})} & 20.6 GB \\
3 & 1-to-many & {30.9 (\textbf{31.3}/30.7/31.1)} & 26.0 GB \\
\multicolumn{2}{c}{~}\\
% \multicolumn{2}{c}{~}\\
\end{tabular}
\end{center}}\end{minipage}
}
\hspace{2em}
%#################################################
% temperature
%#################################################
\subfloat[
\textbf{Temperature $\tau$}. $\tau=0.5$ works the best.
\label{tab:temperature}
]{
\begin{minipage}{0.29\linewidth}{\begin{center}
\tablestyle{4pt}{1.05}
\begin{tabular}{cc}
$\tau$ & AP (r/c/f) \\
\shline
1 & 30.1 (28.4/30.3/30.3)  \\
0.5 & \baseline{\textbf{31.3} (29.4/\textbf{31.7}/\textbf{31.3})} \\
0.15 & 30.8 (\textbf{29.6}/31.0/30.9) \\
0.07 & 29.2 (27.5/29.0/29.6) \\
\end{tabular}
\end{center}}\end{minipage}
}
\hspace{2em}
%#################################################
% contrastive loss weight
%#################################################
\subfloat[
\textbf{Contrastive loss weight $\lambda$}. $\lambda=0.1$ is the optimal.
\label{tab:loss_weight}
]{
\begin{minipage}{0.29\linewidth}{\begin{center}
\tablestyle{4pt}{1.05}
\begin{tabular}{cc}
$\lambda$ & AP (r/c/f)\\
\shline
0.03 & {30.5 (\textbf{29.6/}30.0/31.0)}  \\
0.1 & \baseline{\textbf{31.3} (29.4/\textbf{31.7}/\textbf{31.3})} \\
0.3 & {30.9 (29.4/31.5/30.7)} \\
1 & {28.9 (27.7/28.8/29.3)} \\
\end{tabular}
\end{center}}\end{minipage}
}
%#################################################
\vspace{-.5em}
\caption{\textbf{Ablation experiments for image-text contrastive learning}. The models are based on the Swin-T backbone and trained with O365+CC3M dataset. We report zero-shot \textit{fixed} AP (\%) \cite{dave2021evaluating} on LVIS minival5k \cite{kamath2021mdetr}. r/c/f indicate AP of rare/common/frequent categories, respectively. Default settings are marked in \colorbox{baselinecolor}{gray}. Designs with higher overall AP are selected as our final setting. Baseline of training with only O365 can be referred to the row1 of Table~\ref{tab:train_with_more_datasets}.}
\label{tab:contrastive_ablations} \vspace{-1.5em}
\end{table*}
%###########################################################################################

% effectiveness of deformable head
\begin{table}[t]
\vspace{-.5em}
\centering
\tablestyle{1pt}{1.05}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccc}
\toprule
Pretrain-data & deform & AP (r/c/f) & iter time (s) \\
\midrule
O365 & \xmark & {28.8 (26.0 / 28.0 / 30.0)} & 0.925 \\
O365 & \cmark & {28.6 (24.2 / 27.1 / 30.6)} & 1.075 \\
O365+GoldG+CC3M & \xmark & {37.3 (34.1 / 36.9 / 38.2)} &0.980\\
O365+GoldG+CC3M & \cmark & {\textbf{38.4 (36.7 / 37.9 / 39.1)}} & 1.092\\
\bottomrule
\end{tabular}
}
\vspace{-.7em}
\caption{\textbf{The deformable module} effectively improves the weakly-supervised learning while introducing negligible computational cost. 'iter time' is the training time per iteration.}
\label{tab:deformable_head} \vspace{-.5em}
\end{table}

%##############################################################################################
% training with more data
\begin{table}[t]
\vspace{-.5em}
\centering
\begin{tabular}{lc}
\toprule
Pretrain-data & AP (r/c/f) \\
\midrule
O365 & {28.6 (24.2 / 27.1 / 30.6)} \\
O365+CC3M & {31.3 (29.4 / 31.7 / 31.3)} \\
O365+GoldG+CC3M & {38.4 (\textbf{36.7} / 37.9 / 39.1)} \\
O365+GoldG+CC15M & {\textbf{40.4} (36.0 / \textbf{41.7} / \textbf{40.0)}} \\
\bottomrule
\end{tabular}
\vspace{-.7em}
\caption{\textbf{Incorporating more data from different sources} consistently improves the performance.}
\label{tab:train_with_more_datasets} \vspace{-.5em}
\end{table}

%####################################################################################
% training efficiency
\begin{table}[t]
\vspace{-.5em}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{llcc}
\toprule
Model & Pretrain-data & \makecell{Training time \\ (GPU hours)} & FPS \\
\midrule
GLIP-T \cite{li2021grounded}\dag & O365+GoldG & 7.4k (3.0k)$^\dag$ & 1.6 \\
DetCLIP-T \cite{yao2022detclip} & O365+GoldG+YFCC1M & \textbf{2.0k} & 4.1 \\
DetCLIPv2-T & O365+GoldG+CC15M &  2.1k & \textbf{25.7} \\
\bottomrule
\end{tabular}
}
\vspace{-.7em}
\caption{\textbf{Training efficiency.} For DetCLIP, we directly use the result reported in the paper; while for GLIP, we calculate the training time based on the FPS provided in the paper. $\dag$: 7.4k is calculated based on the official implementation which trains 30 epochs, while 3.0k is obtained by converting it to our setting of 12 epochs.}
\label{tab:training_efficiency} \vspace{-6mm}
\end{table}

%###########################################################################################
% zero-shot performance
\begin{table*}[t]
\vspace{-4mm}
\centering
\begin{tabular}{lllccc}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Detector (Backbone)} & \multirow{2}{*}{Pre-Train Data} & \multicolumn{2}{c}{LVIS}  \tabularnewline
 &  &  & {AP} & {AP$_r$ / AP$_c$ / AP$_f$} \\
\midrule
MDETR \cite{kamath2021mdetr} & DETR\cite{carion2020end} (RN101) & GoldG+ & 24.2 & 20.9 / 24.3 / 24.2   \\ 
\midrule
\gc{Supervised} & \gc{ATSS\cite{zhang2020bridging} (Swin-T)} & \gc{LVIS} & \gc{33.6} & \gc{19.7 / 32.4 / 37.2}  \\
GLIP-T\cite{li2021grounded} & DyHead \cite{dai2021dynamic} (Swin-T)  & O365,GoldG,Cap4M & {26.0} & {20.8 / 21.4 / 31.0}  \\
GLIPv2-T \cite{zhang2022glipv2} & DyHead \cite{dai2021dynamic} (Swin-T) & O365,GoldG,Cap4M & {29.0} & { \ \ \ - \ \ / \ \ \  - \ \ \ / \ \ \ -\ \ \ }   \\
DetCLIP-T \cite{yao2022detclip} & ATSS \cite{zhang2020bridging} (Swin-T) & O365,GoldG,YFCC1M & 35.9 & 33.2 / 35.7 / 36.4   \\
\rowcolor{mypink} DetCLIPv2-T (ours) & ATSS \cite{zhang2020bridging} (Swin-T) & O365,GoldG,CC15M & \textbf{40.4} & \textbf{36.0 / 41.7 / 40.0}  \\
\midrule
\gc{Supervised} & \gc{ATSS\cite{zhang2020bridging} (Swin-L)} & \gc{LVIS} & \gc{43.9} & \gc{30.6 / 43.6 / 46.6}  \\
GLIP-L\cite{li2021grounded} & DyHead \cite{dai2021dynamic} (Swin-L) & O365,GoldG,Cap24M & {37.3} & {28.2 / 34.3 / 41.5}  \\
DetCLIP-L \cite{yao2022detclip} & ATSS \cite{zhang2020bridging} (Swin-L) & O365,GoldG,YFCC1M & 38.6 & 36.0 / 38.3 / 39.3  \\
\rowcolor{mypink}DetCLIPv2-L (ours) & ATSS \cite{zhang2020bridging} (Swin-L) & O365,GoldG,CC15M & \textbf{44.7}  &  \textbf{43.1 / 46.3 / 43.7} \\
\bottomrule
\end{tabular}
\vspace{-.7em}
\caption{\textbf{Zero-shot performance} on LVIS minival5k \cite{kamath2021mdetr}. \textit{Fixed} AP \cite{dave2021evaluating} is reported. DetCLIPv2 achieves SoTA performance.}
\label{tab:main_table} \vspace{-1.2em}
\end{table*}
%##########################################################################################


\subsubsection{Ablations for Image-text Contrastive Learning}
\vspace{-1mm}\label{subsubsec:contrastive_ablation}
We investigate key factors for our image-text contrastive learning to work in Table~\ref{tab:contrastive_ablations}. The experiments are conducted with Swin-T-based model on O365+CC3M datasets.

\paragraph{Proposal selection strategy.} 
Selecting representative regions is critical for image-text contrastive learning. Table~\ref{tab:proposal_selection} studies multiple class-agnostic objectness scores for selecting proposals, which includes foreground classfication score \cite{jjfaster2rcnn} (row1), IoU score \cite{jiang2018acquisition} (row2) and centerness \cite{Tian_fcos} (row3). Except for centerness which is originally designed in ATSS \cite{zhang2020bridging}, other 2 scores are predicted by plugging in an additional head after the regression branch. We consider 3 additional scores to utilize textual information: (1) sample-wised text similarity (row4), i.e., each region calculates the similarities with the textual concepts of the sample and the maximum similarity is used as the objectness score; (2) batch-wised text similarity (row5), i.e., the similarities are calculated between a region and textual concepts within a local batch, as described in Sec.~\ref{contrastive_learning}; and (3) multiplying the batch-wised text similarity with the centerness score (row6), which is commonly adopted by conventional detectors \cite{Tian_fcos,zhang2020bridging}. 

Among 3 class-agnostic objectness scores, centerness and IoU scores are superior to classification score, indicating that localization-based objectness scores provide better class-agnostic proposals. The result is consistent with the observations in \cite{kim2022oln}. Considering only the sample-wised text similarity performs worse than using class-agnostic scores, since the regions selected in this way make it easier to distinguish between positive and negative samples in the contrastive learning, thus reducing the learning efficiency. Batch-wise similarity addresses the problem by considering text similarities with negative samples and achieves the best performance of 31.3 AP. Further integrating centerness score results in a performance drop to 30.9 AP.

\paragraph{Number of proposals $k$.} Table~\ref{tab:number_proposals} investigates the optimal $k$ when selecting proposals. We vary $k$ from 25 to 200. Using a large $k=200$ results in too many low-quality candidates that slightly decreases the performance. A too small $k=25$ leads to insufficient region extraction which causes a noticeable performance drop. A modest design with 100 proposals achieves the best performance.

\paragraph{Contrastive loss design.} Table~\ref{tab:contrastive_loss} performs ablation experiments on different sides of the image-text contrastive loss (Eq.~\ref{eq:contrastive_loss}). 3 designs are considered: (1). only image-to-text side loss; (2) only text-to-image side loss; and (3) bilateral loss. As discussed in Sec.~\ref{contrastive_learning}, using only image-to-text contrastive loss can lead to a significant performance degradation (29.8 AP) due to the \textit{partial labeling} problem of the image-text pair data. Excluding image-to-text contrastive loss can alleviate the problem and achieving a better performance of 31.3 AP. 

\paragraph{Word-region alignment strategy.} Table~\ref{tab:matching_strategy} investigates word-region alignment strategies described in Sec.~\ref{contrastive_learning}. Specifically, for fine-grained word-region alignment, 2 matching strategies are studied: (1) 1-to-1 match (row2), i.e.,  each textual concept is matched with its closest region and (2) 1-to-many match (row3), i.e., each textual concept calculates similarities with all regions, which is then aggregated through a softmax-weighted-sum operation. Besides, we also study a coarse-grained image-text matching strategy proposed in \cite{zhou2022detecting} (row1). Specifically, it directly calculates the similarity between the max-size proposal of image and the entire caption of text. Both fine-grained word-region alignment strategies outperform the coarse-grained image-text alignment. Assigning each textual concept with the closest region reaches the best performance (31.3 AP) and substantially saves the GPU memory compared to the 1-to-many strategy, which allows a larger batch size to boost the contrastive learning.

\paragraph{Temperature and Loss weight.} Table~\ref{tab:temperature} and ~\ref{tab:loss_weight} study the optimal values of temperature $\tau$ in Eq.~\ref{eq:contrastive_loss} and loss weight $\lambda$ in Eq.~\ref{eq:overall_objectives}, respectively. The default values of $\lambda=1,\ \tau=0.07$ commonly adopted in standard constastive learning methods  \cite{radford2021learning,yao2021filip} perform poorly in our case. We use $\tau=0.5$ and $\lambda=0.1$ as our final setting. 

% \subsubsection{Comparison with Related Methods}
\vspace{-4mm}
\subsubsection{Effectiveness of Deformable Module} \label{subsubsec:deformable}
\vspace{-1mm}
Table~\ref{tab:deformable_head} studies the effectiveness of the proposed deformable module described in Sec.~\ref{objective_and_model}. The deformable module effectively promotes the  weakly supervised learning. Specifically, it presents negative effect when trained with strongly supervised detection data (row1 and 2), while demonstrating substantial performance improvement when incorporating grounding/image-text pair data without localization supervisions (row3 and 4). Besides, with only 1 deformable convolution, it introduces negligible computational cost in terms of training time. 

\vspace{-4mm}
\subsubsection{Incorporating More Data Helps Learning}
\vspace{-1mm}
Table~\ref{tab:train_with_more_datasets} reports the performance gains when scaling up the training data. With the proposed framework, incorporating
more training data from different sources can consistently improve the performance. Compared to training with only Objects365, including CC3M effectively improves the overall AP from 28.6 to 31.3, especially for rare categories (from 24.2 to 29.4, +5.2 AP). GoldG helps significantly improve the overall AP to 38.4 thanks to its instance-level annotations. Including CC12M pushes the envelop further, achieving a 40.4 overall AP which already surpasses the performance of the fully-supervised method (see Table~\ref{tab:main_table}).

\vspace{-3mm}
\subsubsection{Training Efficiency} 
\vspace{-1mm}
We develop DetCLIPv2 with several designs that facilitate training efficiency, including using low-resolution inputs for image-text pairs, limiting the maximum token length of the text encoder to 16, etc. Table~\ref{tab:training_efficiency} compares the training efficiency of DetCLIPv2 with that of GLIP \cite{li2021grounded} and DetCLIP \cite{yao2022detclip}. First, both DetCLIP and DetCLIPv2 are more efficient than GLIP due to the lightweight architecture design, as described in Sec.~\ref{objective_and_model}. 
Besides, DetCLIPv2 is much faster than DetCLIP: it exploits 13$\times$ more image-text pairs than DetCLIP with a similar training time, achieving more than 6$\times$ FPS speed up (25.7 FPS v.s. 4.1 FPS). This indicates the great scaling property of our method and allows a possibility of incorporating a larger-scale image-text pairs to build a more powerful open-vocabulary detection system.

%############################################################################################
% word-region alignment
\begin{figure*}[th!]
\vspace{-4mm}
\begin{center}
\includegraphics[width=\textwidth]{figures/word_region_align.pdf}
\vspace{-8mm}
\caption{\textbf{Visualization of word-region alignment}. Image-text pairs in CC12M are used for visualizations. Noun phrases (or textual concepts) in captions are highlighted in bold text and their corresponding matched regions are displayed with the same color. 
}
% patches in the images and words in the sentences.}
\label{fig:word_region_align}
\end{center}
\vspace{-7mm}
\end{figure*}
%############################################################################################
\vspace{-1mm}
\subsection{Main Results}\label{subsec:zero-shot_results}
\vspace{-1mm}
\subsubsection{Zero-shot Performance on LVIS}
\vspace{-1mm}
To compare with the existing works, We train DetCLIPv2 with the best setting reported in~\ref{subsubsec:contrastive_ablation}. We vary models' capacity by considering two backbones, i.e., swin-T and swin-L ~\cite{liu2021swin}, denoted as DetCLIPv2-T/L, respectively. Table~\ref{tab:main_table} reports the comparison with MDETR \cite{kamath2021mdetr}, GLIP \cite{li2021grounded}, GLIPv2 \cite{zhang2022glipv2}, and DetCLIP\cite{yao2022detclip} on zero-shot performance. For better demonstration, we also report the performances of the fully-supervised method on LVIS.

DetCLIPv2 outperforms the existing methods by a large margin. Compared to GLIP/GLIPv2, DetCLIPv2 uses a more lightweight backbone (without heavy DyHead \cite{dai2021dynamic} and cross-modal fusion) but still achieves better performances, e.g., DetCLIPv2-T outperforms GLIP-T/GLIPv2-T by 14.4/11.4 AP, respectively. Compared to DetCLIP, DetCLIPv2 achieves 4.5 (40.4 v.s. 35.9) and 6.1 (44.7 v.s. 38.6) AP performance gains for Swin-T- and Swin-L-based models, respectively. Despite using more training data, our total training cost is on par with DetCLIP \cite{yao2022detclip}, as reported in Table~\ref{tab:training_efficiency}.  \textit{Notably, our models beat their fully-supervised conterparts in a zero-shot manner}, e.g, +6.8/0.8 AP for Swin-T- and Swin-L-based models, respectively. Especially, due to the long-tailed property of LVIS, the improvements over rare categories are significant, i.e., more than 10 AP improvements can be observed on both models.


\vspace{-4mm}
\subsubsection{Transfer Results with Fine-tuning}
\vspace{-1mm}
%#########################################################################################
% full-shot performance
\begin{table}[t]
\vspace{-.5em}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcc}
\toprule
\multirow{2}{*}{Method} & LVIS & ODinW13 \tabularnewline
  & {AP (AP$_{r}$/AP$_{c}$/AP$_{f}$)} & average AP \\
\midrule
GLIP-T \cite{li2021grounded}  & - &  64.9 \\
GLIPv2-T \cite{zhang2022glipv2} & $^\dag$50.6  ( - / - / - )  & 66.5 \\
\rowcolor{mypink} DetCLIPv2-T (ours)  & \textbf{50.7} (44.3/52.4/50.3) & \textbf{68.0} \\
\midrule
GLIP-L \cite{li2021grounded}  & - &  68.9 \\
GLIPv2-B \cite{zhang2022glipv2}  & $^\dag$57.3 ( - / - / - ) &  69.4 \\
GLIPv2-H \cite{zhang2022glipv2}  & $^\dag$59.8 ( - / - / - )  &  \textbf{70.4} \\
\rowcolor{mypink}DetCLIPv2-L (ours)  & \textbf{60.1} (58.3/61.7/59.1) & \textbf{70.4}\\
\bottomrule
\end{tabular}
}
\vspace{-.7em}
\caption{\textbf{Fine-tuning performance}. \textit{Fixed} AP \cite{dave2021evaluating} on LVIS minival5k \cite{kamath2021mdetr} and average AP on ODinW13 \cite{li2021grounded} are reported. Numbers with $^\dag$ mean mask annotation are used for training. }
\label{tab:full-shot_performance} \vspace{-1em}
\end{table}
%#########################################################################################

We study the transferability of DetCLIPv2 by fine-tuning it on down-stream tasks. Specifically, we conduct full-shot fine-tuning on LVIS \cite{gupta2019lvis} with 1203 categories and ODinW13 \cite{li2021grounded,zhang2022glipv2} containing 13 detection tasks. The results are shown in Table~\ref{tab:full-shot_performance}. Without using mask annotation for training, DetCLIPv2 slightly outperforms GLIPv2 on LVIS, e.g., 50.7 AP of DetCLIPv2-T v.s. 50.6 AP of GLIPv2-T. On ODinW13, DetCLIPv2-T demonstrates superior performance compared to GLIP-T/GLIPv2-T, outperforming GLIP-T/GLIPv2-T by 3.1/1.5 average AP, respectively; and DetCLIPv2-L with Swin-L backbone achieves the same performance (70.4 average AP) with GLIPV2-H that uses a heavier Swin-H backbone.

\subsection{Visualizations and Analyses}\label{subsec:analysis_and_discussion}
\vspace{-1mm}
\paragraph{Visualization of word-region alignment.} Figure~\ref{fig:word_region_align} visualizes the learning results of word-region alignment on image-text pairs in CC12M \cite{changpinyo2021cc12m}. For each textual concepts, we find its best matching with the highest similarity to it, as described in Sec.~\ref{contrastive_learning}. Our approach achieves accurate word-region alignment (on instance-level) with great generalization, which is demonstrated by several aspects: (1) it successes to recognize concepts that do not covered by detection datasets, e.g., `parsley' in case (b); (2) it works for images with \textit{natural distribution shifts} \cite{taori2020measuring}, e.g., the sketch image in case (a) and the cartoon image in case (c); and (3) it is capable of resolving co-reference expressions, e.g., the `juvenile' in case (d) refers to `young bird' and `curator' in case (e) refers to a person. These capabilities are critical for open-world detectors but cannot be reflected well in the commonly adopted evaluation benchmarks like LVIS \cite{gupta2019lvis}.

%####################################################################################
% average recall
\begin{table}[t]
\vspace{-.5em}
\centering
\begin{tabular}{lc}
\toprule
Pretrain-data & AR (s/m/l) \\
\midrule
O365 & {44.9 (35.2 / 52.9 / 62.0)} \\
O365+GoldG & {57.2 (42.1 / 67.0 / 76.2)} \\
O365+GoldG+CC15M & {\textbf{59.4 (44.5 / 69.4 / 76.8)}} \\
\bottomrule
\end{tabular}
\vspace{-.7em}
\caption{\textbf{Average recall (AR)} across 0.5-0.95 IoU on LVIS. s/m/l denote for small/medium/large objects, respectively.}
\label{tab:average_recall} \vspace{-1em}
\end{table}
%####################################################################################

\paragraph{Learning from image-text pairs benefits localization.} Table~\ref{tab:average_recall} provides more evidences to show that learning from image-text pairs also helps localization. Specifically, we evaluate the average recall across 0.5-0.95 IoU on LVIS and compare models trained with different data. Incorporating image-text pairs brings a significant and comprehensive recall improvements for small, medium, and large objects, demonstrating the effectiveness of our end-to-end unified training framework.  


